DevFormer: A Symmetric Transformer for Context-Aware Device Placement

In this paper, we present DevFormer, a novel transformer-based architecture for addressing the complex and computationally demanding problem of hardware design optimization. Despite the demonstrated efficacy of transformers in domains including natural language processing and computer vision, their use in hardware design has been limited by the scarcity of offline data. Our approach addresses this limitation by introducing strong inductive biases such as relative positional embeddings and action-permutation symmetricity that effectively capture the hardware context and enable efficient design optimization with limited offline data. We apply DevFoemer to the problem of decoupling capacitor placement and show that it outperforms state-of-the-art methods in both simulated and real hardware, leading to improved performances while reducing the number of components by more than $30\%$. Finally, we show that our approach achieves promising results in other offline contextual learning-based combinatorial optimization tasks.

==> figures/AM_modifications.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{Figures/PNGfiles/AM_modification.png}
    \caption{Comparison of original attention model (AM) and its modified neural architecture in CDML framework.}
    \label{fig:AM_modification}
    \vspace{-4mm}
\end{figure}

==> figures/CDML_complexity.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.75\textwidth]{Figures/PNGfiles/CDML_complexity.png}
    \caption{Overall hardware design complexity reduction when applying CDML.}
    \label{fig:CDML_complexity}
\end{figure}

==> figures/Impedance.tex <==
\begin{wrapfigure}{r}{0.45\textwidth}
  \begin{center}
  \vspace{-8mm}
    \includegraphics[width=0.5\textwidth]{Figures/PDFfiles/figure4.pdf}
    \vspace{-6mm}
    \caption{\label{impedance}An example of impedance suppression after 20 decaps placed by each method.}
    \label{fig:impedance}
    \vspace{-20pt}
  \end{center}
\end{wrapfigure}

==> figures/ablations_main_fede.tex <==
\begin{figure*}[t]
    \centering
    % \vspace{-5mm}
    \begin{subfigure}[t]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/pdf/ablations/Component ablation.pdf}
        % \caption{DevFormer and CSE component analysis}
        \vspace{-6mm}
        \caption{Ablation on \ourmethod{} and CSE.}
        \label{fig:component_ablation}
    \end{subfigure}
    \quad
    \begin{subfigure}[t]{0.31\textwidth}
        \centering
        %\includegraphics[width=\textwidth]{figures/pdf/ablations/expert_data_performance_fede.pdf}
        \includegraphics[width=\textwidth]{figures/pdf/ablations/ablation_b.pdf}
        % \caption{\textcolor{blue}{Offline data-efficiency evaluation ($P=3, \lambda=8$)}}
        \vspace{-6mm}
        \caption{Ablation on \ourmethod{} components \textbf{w/o CSE}.}
        \label{fig:ablation_b}
    \end{subfigure}
    \quad
    \begin{subfigure}[t]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/pdf/ablations/ablation_c.pdf}
        % \caption{\textcolor{blue}{Performance comparison with number of decap variation on HBM}}
        \vspace{-6mm}
        \caption{Ablation on \ourmethod{} components \textbf{with CSE}.}
        \label{fig:ablation_c}
    \end{subfigure}
    \vspace{-2mm}
    \caption{Ablation study on \ourmethod{} architecture and CSE learning scheme. Note that \ourmethod{} architecture is based on AM with newly devised PPE, PCN and RCN, and our method refers to the \ourmethod{} trained with CSE scheme. \fede{figure (c) may be misleading: i think it is better to say: "AM" and "AM w/ CSE". Otherwise one can think that AM already had that good performance.}}
    %(a) Collaborative Symmetricity Exploitation (CSE) improves performance across models. (b) Offline data-efficiency. (c) Pareto front of performance and the number of decaps placed on a real-world high-bandwidth memory: \ourmethod{} shows the best performance while employing the least number of capacitors among baselines.}
    \label{fig:ablations_main_fede}
    % \vspace{-6mm}
\end{figure*}




==> figures/complexity.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.75\textwidth]{Figures/PNGfiles/Overall_hardware_design_complexity.png}
    \caption{Hardware design composed of multi-level tasks and its complexity.}
    \label{fig:complexity}
\end{figure}

==> figures/validation.tex <==
\begin{figure}[b]
    \centering
    \vspace{-2mm}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/PNGfiles/validation.png}
        \caption{\ourmethod{} on AM-IL baseline.}
        \label{figure:ablation_validation}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/PNGfiles/rl_ablation.png}
        \caption{\ourmethod{} on AM-RL baseline.}
        %Comparison with RL baseline to evaluate sample efficiency and performances in training
        \label{figure:rl_ablation}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/PNGfiles/n_ablation.png}
        \caption{\ourmethod{} with $N$ Variation.}
        %Comparison with RL baseline to evaluate sample efficiency and performances in training
        \label{fig:n_ablation}
    \end{subfigure}
    
    
    \caption{Ablation study on \ourmethod{} components}
    \vspace{-6pt}
    \label{figure:ablation}
\end{figure}

==> sections/archive/Rebuttal.tex <==
\subsection{General Comment to the Reviewers}
We would first like to appreciate all your valuable comments. We revised our paper based on your comments and marked them in blue. \textcolor{blue}{In the revised paper, we formally defined the order-bias metric with theoretical analysis of AP-symmetricity (Appendix G). To this end, we provide some reasoning for the loss function design of CSE using a formally defined order-bias metric. Moreover, we report empirical measurement of AP-symmetricity based on the order-bias metric in Appendix H. We expect this revision process can improve the clarity of the method and technical novelty. }

The source codes for DPP benchmark and CSE as well as the baselines will be released to the public after the decision is made. Here we present clarifications to the novelty and contribution of this work. 

\textbf{A novel symmetric learning scheme for contextualized policy.} There exists several works \citet{cohen2016group,thomas2018tensor,fuchs2020se,satorras2021n} that learn various symmetricities of input data in the domain space for regression and classification tasks. However, learning symmetricity in solution space is less studied as learning the symmertrcities in solution space of sequential policy (generative decision) is challenging. \citep{bengio2021flow} tackled solution symmetricity of sequential policy by turning the Markov decision process (MDP) tree model into the directed acyclic graph (DAG)-based flow model. However, they target single-task optimization where the optimal solution set is unchanged. On the other hand, our CSE is an effective solution symmetric learning scheme for the contextualized policy capable of adapting to newly given task-condition.

\textbf{DPP benchmark.} DPP is a widely studied task in hardware domain without public release of the simulation models and source codes for the methods. In this work, by releasing the DPP benchmark with open-source simulation models and our reproduced baselines, DRL-based methods, meta-heuristic methods, behavior cloning-based methods and our state-of-the-art CSE method, we expect huge industrial impacts to the hardware and the ML communities.






\subsection{Response to Reviewer 1PDU}
Thank you for your valuable comments. We'd like to address your comments by providing further explanations and additional experimental results.

\textbf{Responses to the Weaknesses}
\begin{itemize}[leftmargin=1cm]
    \item The paper you referenced is our work-in-progress paper, which has not yet been published. The finalized version is submitted to this ICLR 2023 venue. 
    \item Based on your feedback, we provide extra experimental results for AM-IL and Arb-IL. IL-based methods including CSE were trained with $N=1,000$ offline data. See our revised Figure 8 and section 5.5. We compared the \ourmethod{} to GA\{$M=100$\}, AM-IL and Arb-IL on placing varying number of decaps, $K$, for 100 test cases. \ourmethod{} achieved the highest performance with significantly fewer decaps. For instance, the performance score of 26.68, attained with 40 decaps by GA\{$M=100$\} and 34 decaps by AM-IL, was achieved with only 26 decaps placed by zero-shot \ourmethod{}. Arb-IL was unable to achieve 26.68 even with 80 decaps. Reducing the number of decaps is a huge contribution to the industry as hardware devices are mass-produced, reducing a single decap can greatly reduce production costs and also saves space for other components.
    \item The placement subfigures on figure 1 are intended to be the same. We wanted to emphasise that there exists many trajectories that result in identical placement solution as the order of placement does not matter for hardware placement tasks. Figure 1 elucidates our motivation for designing a policy that is not affected by the order and, at the same time, for reducing solution space. \textcolor{blue}{To improve the clarification of figure 1, we revised the figure at the new manuscript.}
\end{itemize}

\textbf{Novelty and Further Applications}\\
Inducing symmetricities to improve generalization capability of model has widely been practiced in various fields such as point cloud regression and molecule graph. However, such methods induce symmetricity to the input of neural network because they target regression and classification tasks, which do not generate complex solutions. On the other hand, inducing symmetricities to the output solution space of neural network is less explored and is very challenging.

Placement tasks such as our DPP find solutions from combinatorial space. Thus, auto-regressive schemes were widely implemented due to its capability of processing a high-dimensional input. However, auto-regressive schemes incur unwanted inductive bias because sequentially generating solution leads to unwanted bias in terms of the order of placement.

GflowNet was proposed to overcome the limitation in molecular generation task by inducing solution symmetricities. However, GflowNet optimizes a single task while DPP requires a task-conditioned contextualized policy (i.e., optimizing infinite tasks with different conditions). Our CSE allows training of a task-conditioned contextualized policy while inducing solution symmetricities to improve sample efficiency of training and generalization capability of the trained policy. 

Though we only applied to DPP, the proposed CSE can be applied to various applications including chip placement, via placement, floor planning, robot assignment and set covering as long as sufficient expert offline data is available.


\subsection{Response to Reviewer XtSs}
Thank you for your valuable comments. We'd like to address your comments by providing further explanations.

\textbf{Regarding DPP Benchmark}\\
We admit that DPP is not something ML community is familiar with and we know there exists well-explored benchmarks that are worth solving. However, DPP is a new type of task and has distinct characteristics that widely-solved benchmarks do not have and characteristics that are shared with various real-world problems, especially hardware problems. 

Characteristics of DPP benchmark are:
\begin{itemize}[leftmargin=1cm]
    \item Objective evaluation and data generation are costly in terms of time and computation; less iteration preferred and high sample-efficiency required.
    \item Task condition is determined by higher-level task and is changing; a task-conditioned contextualized policy (i.e., solver) capable of producing solutions to changing problem conditions by zero-shot inference is necessary.
    %\item Each task is a combinatorial optimization problem that finds solutions from combinatorial space.
\end{itemize}

Although we applied our method to a specific problem (i.e., DPP), the novelty of our method CSE lies mainly on designing the learning procedure and neural architecture considering the task characteristics to improve sample efficiency and generalization capability. In fact, many tasks in hardware domain, such as chip placement, via placement and routing, share characteristics mentioned above and thus require ML methodologies. CSE is applicable to any placement task as long as sufficient expert offline data is available.

%Our CSE overcomes the overfitting issue of imitation learning with offline data by inducing action-permutation (AP)-symmetricity and allows sample-efficient offline training of a task-conditioned policy.

\textbf{Reproducibility}\\
We will open our source codes for CSE and the DPP benchmark public after decision is made. We will encourage researchers in the ML community to further engage in solving DPP benchmark to develop various algorithms applicable to real-world problems.

\textbf{Technical Novelty}\\
% The novelty of CSE is summarized as:
% \begin{itemize}[leftmargin=1cm]
%     \item Regularization through solution symmetricity learning.
%     \item Inducing AP-symmetricity through both imitation learning (i.e., behavior cloning) and consistency learning (i.e., self-supervised learning).
% \end{itemize}

\textcolor{blue}{To clarifies the technical novelty of our loss scheme, we formally introduced the order-bias metric to measure AP-symmetricity in the revised manuscript. The order bias is a general property of a sequential solution generation scheme. It measures how much the solver has different probabilities to generate AP-symmetric solutions. We theoretically proved that AP-symmetricity is satisfied when order bias becomes zero (Theorem 3.1).} 

\textcolor{blue}{Our loss scheme is specifically designed to reduce the order bias based upon theoretical proof that the designed loss term guarantees AP-symmetricity. Therefore, our technical novelty comes from designing a proper loss scheme using the theoretical analysis, not from applying self-supervised learning.
}

% Our method is not based on policy gradient reinforcement method. CSE is a solution symmetricity learning method based on behavior cloning (i.e., imitation learning). Our CSE overcomes the over-fitting issue of imitation learning with offline data by inducing action-permutation (AP)-symmetricity and allows sample-efficient offline training of a task-conditioned policy. Moreover, the self-generated labels also induces AP-symmetricity to further improve the generalization capability.

% Inducing symmetricities to improve generalization capability of model has widely been practiced in various fields such as point cloud regression and molecule graph. However, such methods induced symmetricity to the input of neural network because they target regression and classification tasks, which do not generate complex solutions. On the other hand, inducing symmetricities to the output solution space of neural network is less explored and is very challenging.

% Placement tasks such as our DPP find solutions from combinatorial space. Thus, auto-regressive schemes were widely implemented for high generalization capability. However, auto-regressive schemes incur unwanted inductive bias because sequentially generating solution leads to unwanted bias in terms of the order of placement.

% GflowNet was proposed to overcome the limitation in molecular generation task by inducing solution symmetricities. However, GflowNet optimizes a single task while DPP requires a task-conditioned contextualized policy (i.e., optimizing infinite tasks with different conditions). Our CSE allows training of a task-conditioned contextualized policy while inducing solution symmetricities to improve sample efficiency of training and generalization capability of the trained policy. 

% Though we only applied to DPP, the proposed CSE can be implemented to various applications including chip placement, via placement, floor planning, robot assignment and set covering as long as sufficient expert offline data is available.

\textbf{State-of-the-art Performance and Baselines}\\
According to the experimental results, our CSE achieved state-of-the-art performance. We reproduced the baseline methods published in top-tier journals in hardware domain for comparison. The baselines are obviously not considered weak. We'd like to emphasize that the zero-shot performance of pre-trained policy shows a greater performance on unseen problems than highly iterative search-based meta heuristic methods. As shown in Table 1, our CSE takes 500 less simulations per given problem and still outperforms GA.  


\subsection{Response to Reviewer PJWA}
Thank you for your valuable comments. We'd like to address your comments by providing further explanations and additional experimental results.

\textbf{Response to the Weaknesses}
\begin{itemize}
    \item Our CSE is applicable to any placement problem, where the order of placement does not affect the overall performance. We define placement design task as assigning components to generate final design. For instance, when we were given furniture placement task, the final design is what matters rather than in what order the furniture were placed. If the order of placement matters, the task is rather considered a scheduling or routing problem such as TSP.
    \item We conducted additional experiments on sample-efficiency of Arb-IL and reported in revised Figure 6. Since the sample refers to offline data, we only compared with IL-based baselines. As a result, CSE was proven most sample-efficient (i.e., showed highest performance with much less offline data) out of IL methods. Furthermore, the performance of AM-IL and Arb-IL saturated at $N=500$ while the performance of CSE continuously increased with $N$.
    % \item The novelty of the proposed method is focused on training with limited offline data and training a task-conditioned contextualized solver capable of solving changing task conditions. 
\end{itemize}

\textbf{Technical Novelty}\\
% The novelty of CSE is summarized as:
% \begin{itemize}[leftmargin=1cm]
%     \item Regularization through solution symmetricity learning.
%     \item Inducing AP-symmetricity through both imitation learning (i.e., behavior cloning) and consistency learning (i.e., self-supervised learning).
% \end{itemize}

\textcolor{blue}{Learning symmetricity on combinatorial space is important and difficult. To achieve AP-symmetricity (which is the general symmetric nature of placement tasks), we proposed a simple and novel loss scheme, which gives both empirical powerful performances and theoretical analysis.}

\textcolor{blue}{To clarifies the technical novelty of our loss scheme, we formally introduced the order-bias metric to measure AP-symmetricity in the revised manuscript. The order bias is a general property of a sequential solution generation scheme. It measures how much the solver has different probabilities to generate AP-symmetric solutions. We theoretically proved that AP-symmetricity is satisfied when order bias becomes zero (Theorem 3.1).} 

\textcolor{blue}{Our loss scheme is specifically designed to reduce the order bias based upon theoretical proof that the designed loss term guarantees AP-symmetricity. Therefore, our technical novelty comes from designing a proper loss scheme using the theoretical analysis, not from applying self-supervised learning.}


\textbf{Empirical Evaluation and Perturbation Analysis}\\
Empirical evaluation of the proposed method in terms of power noise reduction on high bandwidth memory in comparison to baseline method is reported in Appendix E. Sensitivity analysis on hyperparameters are provided in Appendix F.



\subsection{Response to Reviewer 1Sai}
Thank you for your valuable comments. We revised our manuscript according to your comments.

\textbf{Response to the Weaknesses}
\begin{itemize}[leftmargin=1cm]
    \item We revised Figure 2 and 4 in the main paper.
    \item We also revised section 5.2 of the main paper based on your comment. CSE was capable of extrapolation over low-quality offline data due to the following reasons. \textcolor{blue}{First, an general context about AP-symmetricity was explicitly given to the model. Second, contextualized neural architecture was capable to extract major context to determine DPP performances. Lastly, policy generates a solution with high confidence (with greedy rollout) based on extracted context.} 
    \item Typo in Figure 1 is corrected.
\end{itemize}

==> tables/AM_modifications.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/png/AM_modification.png}
    \caption{Comparison of original attention model (AM) and its modified neural architecture in CDML framework.}
    \label{fig:AM_modification}
    \vspace{-4mm}
\end{figure}

==> tables/CDML_complexity.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.75\textwidth]{figures/png/CDML_complexity.png}
    \caption{Overall hardware design complexity reduction when applying CDML.}
    \label{fig:CDML_complexity}
\end{figure}

==> tables/Components.tex <==
\begin{table}[t]
\fontsize{9}{9}\selectfont
\begin{center}
\caption{Ablation study on CSE components trained with $N=100$ (the higher the better).}
\label{components}
\begin{tabular}{lcc}
\specialrule{1.0pt}{0pt}{4pt}
& Validation Score & Test Score\\
\specialrule{0.5pt}{0pt}{4pt}
AM-IL (baseline policy) & 11.49 &10.93 \\
+ Meta Learner& 12.28 &12.01 \\
+ Expert Exploitation & 12.69 &12.48 \\
+ Expert Exploitation + Self Exploitation& 12.78  &12.50\\
+ Meta Learner + Expert Exploitation & 12.97 &12.73  \\
+ Meta Learner + Expert Exploitation + Self-Exploitation (\ourmethod{}) & \textbf{12.98} &\textbf{12.73} \\
\specialrule{1.0pt}{0pt}{4pt}
\end{tabular}
\end{center}
\vspace{-8mm}
\end{table}

==> tables/DPP.tex <==



\begin{figure}[h]
    \centering
    \vspace{-3mm}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/figure3.pdf}
        \caption{Unit-cell representation of target PDN of an IC.}
        \label{figure:DPP(a)}
    \end{subfigure}
    \hspace{20pt}
        \begin{subfigure}[b]{0.37\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/figure3_b.pdf}
        \caption{Z-parameter of target PDN.}

        \label{fig:DPP(b)}
    \end{subfigure}
    
    \caption{Unit-cell and Z-parameter representations of real-world target PDN.}
    \label{DPP}\
    \vspace{-4mm}
\end{figure}

==> tables/GA_additional.tex <==
\begin{table}[h!]
\fontsize{9}{9}\selectfont
\begin{center}
\caption{{Ablation study on genetic algorithm with different operator values.}}
\label{Table01}
\begin{tabular}{cccc}
\specialrule{1.0pt}{0pt}{4pt}
PI Simulation ($M$) & Population Size ($P$) & Generations ($G$) & Avg. Score\\
\specialrule{1.0pt}{0pt}{4pt}
\begin{tabular}{c}
\multirow{3}{*}{1000}
\end{tabular}
& 50 & 20 & 12.61\\
& 100 & 10 & 12.82\\
& 200 & 5 & 12.79\\

\specialrule{0.5pt}{0pt}{4pt}
\begin{tabular}{c}
\multirow{4}{*}{2000}
\end{tabular}

& 50 & 40 & 12.37\\
& 100 & 20 & 12.84\\
& 200 & 10 & 12.83\\
& 400 & 5 & 12.80\\

\specialrule{1.0pt}{0pt}{4pt}
\end{tabular}
\end{center}
\vspace{-2mm}
\end{table}

==> tables/Impedance.tex <==
\begin{wrapfigure}{r}{0.45\textwidth}
  \begin{center}
  \vspace{-8mm}
    \includegraphics[width=0.5\textwidth]{figures/figure4.pdf}
    \vspace{-6mm}
    \caption{\label{impedance}An example of impedance suppression after 20 decaps placed by each method.}
    \label{fig:impedance}
    \vspace{-20pt}
  \end{center}
\end{wrapfigure}

==> tables/complexity.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.75\textwidth]{figures/png/Overall_hardware_design_complexity.png}
    \caption{Hardware design composed of multi-level tasks and its complexity.}
    \label{fig:complexity}
\end{figure}

==> tables/encoder-decoder.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\textwidth]{figures/figure2_revised.png}
    \vspace{-2mm}
    \caption{\textcolor{red}{Illustration of collaborative distillation process. } }
    \vspace{-5mm}
    \label{fig:distillation}
\end{figure}

==> tables/main_figure1.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/figure1_revised.png}
    \caption{Overall procedure of the proposed collaborative distillation meta learning (CDML)}
    \label{fig:main_figure}
    \vspace{-4mm}
\end{figure}

==> tables/validation.tex <==
\begin{figure}[b]
    \centering
    \vspace{-2mm}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/png/Validation.png}
        \caption{CDML on AM-IL baseline.}
        \label{figure:ablation_validation}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/png/rl_ablation.png}
        \caption{CDML on AM-RL baseline.}
        %Comparison with RL baseline to evaluate sample efficiency and performances in training
        \label{figure:rl_ablation}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/n_ablation.png}
        \caption{CDML with $N$ Variation.}
        %Comparison with RL baseline to evaluate sample efficiency and performances in training
        \label{fig:n_ablation}
    \end{subfigure}
    
    
    \caption{Ablation study on CDML components}
    \vspace{-6pt}
    \label{figure:ablation}
\end{figure}
